ReX: A Framework for Incorporating Temporal Information in Model-Agnostic Local Explanation Techniques

Existing local model-agnostic explanation techniques are ineffective for machine learning models that consider inputs of variable lengths, as they do not consider temporal information embedded in these models. To address this limitation, we propose \textsc{ReX}, a general framework for incorporating temporal information in these techniques. Our key insight is that these techniques typically learn a model surrogate by sampling model inputs and outputs, and we can incorporate temporal information in a uniform way by only changing the sampling process and the surrogate features. We instantiate our approach on three popular explanation techniques: Anchors, LIME, and Kernel SHAP. To evaluate the effectiveness of \textsc{ReX}, we apply our approach to six models in three different tasks. Our evaluation results demonstrate that our approach 1) significantly improves the fidelity of explanations, making model-agnostic techniques outperform a state-of-the-art model-specific technique on its target model, and 2) helps end users better understand the models' behaviors.

==> figures/LIME_intro.tex <==
\begin{figure}
    \centering
    \begin{tabular}{@{}l@{\ }l}
        \textbf{Input sentence}:& Bob is not a bad boy. \\
        \textbf{Network output}: & Positive  \\
             \textbf{Explanations}:&\\

    \end{tabular}
    \begin{tabular}{r@{}l}
  \includegraphics[scale=0.345]{figs/lime1}  &
  \includegraphics[scale=0.345]{figs/lime2.pdf}
  % (a) & (b)
                     % \multicolumn{2}{c}{(a)} & \multicolumn{2}{c}{(b)} 
    \end{tabular}
    % \begin{tabular}{@{}rl}
    %     \textbf{Input sentence}: & I hate that man but love her.\\
    %     \textbf{Network output}: & Positive  \\
    %          \textbf{Explanations}:\\
    %          \includegraphics*[scale = 0.33]{figs/LIME-3.pdf} & \includegraphics*[scale = 0.33]{figs/LIME-4.pdf} \\
    %                  \multicolumn{1}{c}{(a)} & \multicolumn{1}{c}{(b)}
    % \end{tabular}
    \caption{Example explanations generated by LIME (left) and \toolname-augmented LIME (right).}
    \label{fig:example2}
\end{figure}

==> figures/ablation.tex <==
\begin{figure*}[t]
    \centering
        % \begin{tabular}{c}
        \includegraphics[scale = 0.34]{figs/ablation.pdf} 
        
        % \includegraphics[scale = 0.25]{figs/ablation_AUROC.png}\\
        % (a) Anchors* vs. Anchors &        (b) LIME* vs. LIME
    % \end{tabular}
    
\caption{Average accuracy and AUROC of explanations for the four sentiment analysis models under different settings. The explanations are generated by LIME and its three augmented versions, which are augmented by \toolname, \toolname without 1D-predicates, and \toolname without 2D-predicates.
}
\label{fig:ablation}
\end{figure*}

% \begin{figure}[t]
%     \centering
%         \begin{tabular}{c}
%         \includegraphics[scale = 0.25]{figs/ablation_acc.png} 
        
%         \includegraphics[scale = 0.25]{figs/ablation_AUROC.png}\\
%         % (a) Anchors* vs. Anchors &        (b) LIME* vs. LIME
%     \end{tabular}
    
% \caption{Fidelity results of the ablation study for illustrating the effect of 1-D and 2-D predicates.}
% \label{fig:ablation}
% \end{figure}

==> figures/anomaly_intro.tex <==

\begin{figure}[t]
    \centering
    \includegraphics[scale=0.28]{figs/Anomaly_exp.pdf}
    \caption{Explaining an anomaly detection RNN with Anchors
and \toolname-augmented Anchors (Denoted as Anchors*). Anchors Explanation: if the values of $x_{414}, x_{417}, x_{416}, x_{416}, x_{418}, x_{413}, x_{419}, x_{412}$ keep, $x_{428}$ will be classified as an anomaly. Anchors* Explanation: if the values of $x_{413}$ and $x_{425}$ keep, and at least 3 data points between them remain, $x_{428}$ will be classified as an anomaly.}
    \label{fig:adexp}
\end{figure}

==> figures/pipeline.tex <==
\begin{figure*}[t]
    \centering
     \includegraphics[scale = 0.38]{figs/pipeline4.pdf}
    \caption{The workflow of generating explanations by a local model-agnostic explanation technique.}
    \label{fig:pipe}
\end{figure*}


==> tables/LIME_SHAP.tex <==
\begin{table}[t]
    \centering
    \caption{Fidelity results (indicated by average precision and coverage) of Anchors}
    \label{table:sound}
    {
        % \small
    \setlength{\tabcolsep}{5pt}
    \begin{tabular}{r@{\vline}c}
        \begin{tabular}{l|c|c|c|c|c}
            \hline
            &\multicolumn{5}{c}{Accurracy(\%)}\\
            \hline
            \multirow{2}{*}{Method} & \multicolumn{4}{c|}{Sentiment Analysis} & Anom. \\
            \cline{2-5}
            & LSTM  & BERT & T5 & GPT-2 & RNN \\ 
            \hline
            LIME  & & 23.6 & 33.9 & \\
            LIME*  & & 48.5 & 64.2 & \\
            \hline
            KSHAP  & & & &  \\
            KSHAP*  & & & & \\
            \hline
        \end{tabular}
         &
        \begin{tabular}{c|c|c|c|c}
            \hline
            \multicolumn{5}{c}{AUROC} \\
            \hline
            \multicolumn{4}{c|}{Sentiment Analysis} &Anom.\\
                \cline{1-4}
             LSTM  & BERT & T5 & GPT-2 & RNN \\ 
            \hline & & & &  \\
                 & & & &  \\
            \hline
                & & & &  \\
                & & & &  \\
            \hline
        \end{tabular}
    \end{tabular}
    }
    \label{table:lime_fidelity}
    \end{table}
    

==> tables/anchor_intro.tex <==
% \begin{table}
%     \centering
%     \caption{Example anchor explanations (a) and \toolname-augmented anchor explanations (b).}
%     {\small
%     \begin{tabular}{c|c|c}
%         % \multicolumn{2}{c|}{} & Input Sentence I & Input Sentence II \\
%         \hline
%         \multicolumn{2}{c|}{\textbf{Input Sentence} } & I. He never fails in any exam. \\
%         \hline
%         \multicolumn{2}{c|}{\textbf{Network output}} & Positive \\
%         \hline
%         \multirow[c]{2}{*}{\textbf{Explanations:}} & (a) & \{never, fails\}  \\
%         \cline{2-3} 
%         & \multirow{2}{*}{(b)} &  \{never, fails\}   \\
%         & & $\wedge\ \text{Pos}_{\text{fails}} - \text{Pos}_{\text{never}} = 1$ \\
%         \hline
%         \multicolumn{2}{c|}{\multirow{2}{*}{\textbf{Input Sentence} } } & II. He never attends any lecture,\\
%         \multicolumn{1}{c}{}& & so he fails in any exam. \\
%         \hline
%         \multicolumn{2}{c|}{\textbf{Network output}}  & Negative\\
%         \hline
%         \multirow[c]{2}{*}{\textbf{Explanations:}} & (a) &  \{never, fails\}  \\
%         \cline{2-3}
%         & \multirow{2}{*}{(b)} &  \{never, fails\}   \\
%         & & $\wedge\ \text{Pos}_{\text{fails}} - \text{Pos}_{\text{never}} \geq 2$\\
%         \hline
%     \end{tabular}
%     }
%     % \add[10pt]
%     \label{tab:example1}
% \end{table}



\begin{figure}
    \centering
  \includegraphics[scale=0.45]{figs/example1_c.pdf} 
    \caption{Example Anchors explanations (a) and REX-augmented Anchors explanations (b).}
    \label{fig:example1new}
\end{figure}

==> tables/anchors.tex <==
\begin{table}[t]
    \centering
    \caption{Fidelity results (indicated by average precision and coverage) of Anchors}
    {
        % \small
    \setlength{\tabcolsep}{5pt}
    \begin{tabular}{r@{\vline}c}
        \begin{tabular}{l|c|c|c|c|c}
            \hline
            &\multicolumn{5}{c}{Precision (\%)}\\
            \hline
            \multirow{2}{*}{Method} & \multicolumn{4}{c|}{Sentiment Analysis} & Anom. \\
            \cline{2-5}
            & LSTM  & BERT & T5 & GPT-2 & RNN \\ 
            \hline
            Anchors &  93.6 & 91.1 & \textbf{97.9} & 98.6 & \textbf{99.3}\\
            Anchors* & \textbf{95.8} & \textbf{94.0} & 97.9 & \textbf{99.8} & 93.5  \\
            \hline
        \end{tabular}
         &
        \begin{tabular}{c|c|c|c|c}
            \hline
            \multicolumn{5}{c}{Coverage (\%)} \\
            \hline
            \multicolumn{4}{c|}{Sentiment Analysis} &Anom.\\
                \cline{1-4}
             LSTM  & BERT & T5 & GPT-2 & RNN \\ 
            \hline
              5.1 & 5.7 & 7.6 & 5.9 & 4.6
            \\ \textbf{12.3} & \textbf{14.2} & \textbf{10.0} & \textbf{10.4} & \textbf{8.7} \\
            \hline
        \end{tabular}
        
    \end{tabular}
    }
    \label{table:anchors_fidelity}
    \end{table}
    

==> tables/comp.tex <==
\begin{table}[t]

    \centering
    \caption{Detailed statistics of the completeness results. ``*'' indicates the version with \toolname.}
    \label{table:completeness_detail}
    {
        % \small
     \begin{tabular}{l|c|c|c|c}
         \hline
         
         \multicolumn{2}{c|}{\multirow{2}{*}{Coverage}} &\multicolumn{3}{c}{Anchors}\\
         \cline{3-5}
            \multicolumn{2}{c|}{} & 10\% & Median & \ 90\% \\
         \hline
         \multirow{2}{*}{RNN-senti.}  &  &  0.6\% &5.0\% & 11.1\%  \\
         \cline{2-5}
                                     & * & 1.8\% &14.6\% &19.5\% \\
         
         \hline
         \multirow{2}{*}{RNN-anom.}  &  & 0.4\% &3.9\% &9.5\%  \\
         \cline{2-5}
                                    & * & 5.8\% &9.8\% &10.5\% \\
        \hline
         \multirow{2}{*}{Transformer}  &  & 1.1\% &5.0\% &11.1\%\\
         \cline{2-5}
                                      & * & 2.5\% &16.3\% &19.1\% \\
         \hline
     \end{tabular}
     }
    \end{table}

==> tables/fidelity.tex <==
\begin{table*}[t]
    \centering
    {
    \setlength{\tabcolsep}{1mm}
    \renewcommand{\arraystretch}{0.9}
    \small
    % \resizebox{1.5\columnwidth}{!}{
    \begin{tabular}{@{}lcccccccccccc@{}}
        \toprule
        \multirow{2}{*}{Method} & \multicolumn{6}{c}{Precision (\%)} & \multicolumn{6}{c}{Coverage (\%)} \\
        \cmidrule(lr){2-7} \cmidrule(l){8-13}
       & LSTM & BERT & T5 & GPT-2 & Llama 2 & Anom. & LSTM & BERT & T5 & GPT-2 & Llama 2 & Anom. \\
       \midrule
       Anchor & 84.74 & 82.64 & 81.74 & 82.03 & 79.15 & 90.40 &1.87 & 2.46 & 1.29 & 8.08 & 1.75 & 4.60 \\
       Anchor* &  86.48 & 84.04 & 84.04 & 82.54 & 80.20 & 89.10 & 10.77 & 12.07 & 11.78 & 10.26 & 10.35 & 8.70\\
       \bottomrule
    \end{tabular}
    }
    % }
    \caption{Average precision and coverage of anchors and ReX-augmented anchors(denoted as anchors*) for sentiment analysis models and the anomaly detection RNN (Anom.).}.
    \label{table:fidelity-anchor}
\end{table*}



\begin{table*}[t]
    \centering
    {
    \setlength{\tabcolsep}{1mm}
    \renewcommand{\arraystretch}{0.9}
    \small
    % \resizebox{1.5\columnwidth}{!}{
   \begin{tabular}{@{}lcccccccccccc@{}}
        \toprule
        \multirow{2}{*}{Method} & \multicolumn{6}{c}{Accuracy (\%)} & \multicolumn{6}{c}{AUROC}\\
        \cmidrule(lr){2-7} \cmidrule(l){8-13}
        & LSTM & BERT & T5 & GPT-2 & Llama-2 &Anom. & LSTM & BERT & T5 & GPT-2 & Llama-2 &Anom. \\
        \midrule
        LIME & 58.47 & 55.78 & 66.66 & 51.46 & 54.35 & 62.30 & 0.604 & 0.584 & 0.603 & 0.533 & 0.521 & 0.575 \\
        LIME* & 75.09 & 68.20 & 86.99 & 69.03 & 62.68 & 80.10 & 0.887 & 0.927 & 0.924 & 0.759 & 0.728 & 0.763\\[0.5em]
        % \midrule
        KSHAP & 63.64 & 58.02 & 66.24 & 56.06 & 51.06 & 62.90 & 0.613 & 0.593 & 0.590 & 0.578 & 0.536 & 0.557\\
        KSHAP* & 86.10 & 83.75 & 73.62 & 69.34 & 61.81 & 77.40 & 0.879 & 0.890 & 0.909 & 0.711 & 0.680 & 0.716\\[0.5em]
        % \midrule
        DecompX & -- & 60.80  &--  & -- & -- & -- & -- & 0.601 & -- & -- &-- &-- \\
        \bottomrule
    \end{tabular}
    }
    % }
    \caption{Average accuracy and AUROC of the explanations generated by LIME, KSHAP, their \toolname-augmented versions, and DecompX for sentiment analysis models and the anomaly detection RNN (Anom.).
}
    \label{tab:fidelity-attr}
\end{table*}


% \begin{table*}[t]
%     \centering
%     \caption{Fidelity results.}
%     {\small
%     \setlength{\tabcolsep}{5pt}
%     \begin{tabular}{r@{\vline}c}
%         \begin{tabular}{l|c|c|c|c|c}
%             \hline
%             \multirow{3}{*}{Method} & \multicolumn{4}{c|}{Sentiment Analysis} & Anom. \\
%             \cline{2-5}
%             & LSTM  & BERT & T5 & GPT-2 & RNN \\ 
%             \cline{2-6}
%             &\multicolumn{5}{c}{Precision (\%)}\\
%             \hline
%             Anchors &  93.6 & 91.1 & \textbf{97.9} & 98.6 & \textbf{99.3}\\
%             Anchors* & \textbf{95.8} & \textbf{94.0} & 97.9 & \textbf{99.8} & 93.5  \\
%             \hline
%             &\multicolumn{5}{c}{Accuracy(\%)}\\
%             \hline
%             LIME   &48.8 & 57.2 & 56.8 & 54.7 & 62.3 \\
%             LIME*   &\textbf{67.9} & \textbf{86.0} &\textbf{ 81.0} & \textbf{66.3} & \textbf{80.1}\\
%             \hline
%             KSHAP  &49.8 & 58.9 &          37.0 &48.1 & 62.9  \\
%             KSHAP*  &\textbf{74.2}  & \textbf{64.1} & \textbf{69.0} &\textbf{61.1} & \textbf{77.4} \\
%             \hline
%         \end{tabular}
%          &
%         \begin{tabular}{c|c|c|c|c}
%             \hline
%             \multicolumn{4}{c|}{Sentiment Analysis} &Anom.\\
%                 \cline{1-4}
%              LSTM  & BERT & T5 & GPT-2 & RNN \\ 
%             \hline
%             \multicolumn{5}{c}{Coverage (\%)} \\
%             \hline
%               5.1 & 5.7 & 7.6 & 5.9 & 4.6
%             \\ \textbf{12.3} & \textbf{14.2} & \textbf{10.0} & \textbf{10.4} & \textbf{8.7} \\
%             \hline
%             \multicolumn{5}{c}{AUROC} \\
%             \hline
%              0.505& 0.519& 0.505 & 0.513 &  0.575\\
%                  \textbf{0.713} &\textbf{0.794 }&\textbf{0.646} &\textbf{ 0.648} &  \textbf{0.763}\\
%             \hline
%                 0.493 & 0.514 & 0.521 &0.577  & 0.557\\
%                 \textbf{0.603} & \textbf{0.682} & \textbf{0.652} &\textbf{0.687} &  \textbf{0.716}\\
%             \hline
%         \end{tabular}
%     \end{tabular}
%     }
%     \label{table:fidelity}
%     \end{table*}
    

==> tables/generative_fidelity.tex <==
\begin{table}[t]
\centering
    {
    \setlength{\tabcolsep}{1mm}
    % \renewcommand{\arraystretch}{0.99}
    \small
    % \resizebox{\columnwidth}{!}{
\begin{tabular}{@{}lcccccc@{}} 
\toprule
Method & \text{LIME} & \text{C-LIME} & \text{LIME*}  & \text{KSHAP} & \text{L-SHAP}& \text{KSHAP*} \\
\midrule
MSE &0.187& 0.137 &0.054&0.069& 0.065 &0.028\\ 
\bottomrule
\end{tabular}
}
% }
\caption{Average mean square error (MSE) of explanations for LLama 2 on the text generation task.}
\label{tab:gene}
\end{table}

==> tables/res_others.tex <==
% \begin{table}[t]
%     \centering
%     \caption{Fidelity results of applying \toolname+KSHAP, DecompX to explain  BERT.}
%     {\small
% \begin{tabular}{@{}lcc@{}}
%         \toprule
%         &KSHAP*  & DecompX  \\
%         \midrule
% Accuracy (\%) & 83.75 & 60.80 \\
% AUROC & 0.890 & 0.601    \\
%         \bottomrule
% \end{tabular}
% \label{table:other}
%     }
%     \end{table}

% \begin{table}[t]
%     \centering
%     \caption{Fidelity results of Using \toolname+KSHAP, DecompX and IG to explain a BERT.}
%     \label{table:user_study}
%     {\small
% \begin{tabular}{l|c|c|c}
%         \hline
%         &KSHAP*  & DecompX  & windowSHAP \\
%         \hline
% Accuracy (\%) & 83.75 & 60.81 & 52.14 \\
% \hline
% AUROC & 0.890 & 0.601 & 0.517   \\

% \hline
% \end{tabular}
% \label{table:other}
%     }
%     \end{table}

==> tables/sound.tex <==
\begin{table}[t]
    \centering
    \caption{Soundness results (indicated by average precision), completeness results (indicated by average coverage), and average executing times.}
    \label{table:sound}
    {
        % \small
    \setlength{\tabcolsep}{5pt}
    \begin{tabular}{l@{\vline}c@{\vline}c}
        
        \begin{tabular}{l|c|c|c}
            \hline
            &\multicolumn{3}{c}{Precision (\%)}\\
            \hline
            \multirow{2}{*}{Method} & \multicolumn{2}{c|}{RNN} & \multirow{2}{*}{Trans.}\\
            \cline{2-3}
            & Senti.  & Anom. &\\
            \hline
            Anchors &          93.5  & \textbf{99.3}           &         91.1  \\
            Anchors* & \textbf{95.8} &         93.5            & \textbf{94.0} \\
            \hline
            LIME & 75.4 & 75.3 & 80.1  \\
            LIME* & \textbf{80.1} & \textbf{88.1} & \textbf{95.6}\\
            \hline
        \end{tabular}
         &
        \begin{tabular}{c|c|c}
            \hline
            \multicolumn{3}{c}{Coverage (\%)} \\
            \hline
            \multicolumn{2}{c|}{RNN} & \multirow{2}{*}{Trans.}\\
                \cline{1-2}
            Senti.  & Anom. &\\
            \hline
                    5.1   &           4.6   &   5.7 \\
            \textbf{12.3} &    \textbf{8.7} &\textbf{14.2} \\
            \hline
                10.0            &    8.2          & 10.0  \\
                \textbf{46.3}       &   \textbf{30.7}  &\textbf{51.1} \\
            \hline
        \end{tabular}
        &
        \begin{tabular}{c|c|c}
            \hline
            \multicolumn{3}{c}{Time (seconds)}\\
            \hline
            \multicolumn{2}{c|}{RNN} & \multirow{2}{*}{Trans.}\\
                \cline{1-2}
            Senti.  & Anom. &\\
            \hline
              \textbf{48.3} &           665.3   &  \textbf{63.1} \\
             77.2 &    \textbf{476.4} &86.0 \\
            \hline
             \textbf{24.9}            &    \textbf{605.2}            & \textbf{205.5}   \\
             42.5       &   824.2            & 248.3\\
            \hline
        \end{tabular}
    \end{tabular}
    }
    \label{table:completeness}
    \end{table}
    

==> tables/time.tex <==
\begin{table*}[t]
    \centering
    {
        \small
    \setlength{\tabcolsep}{1mm}
    % \renewcommand{\arraystretch}{0.9}
    % \resizebox{1.5\columnwidth}{!}{
\begin{tabular}{@{}lcccccccccccccc@{}}
    \toprule
        % & \multicolumn{10}{c}{Sentiment Analysis} & \multicolumn{2}{c}{Anomaly Detection}\\
        % \cmidrule(lr){2-11} \cmidrule(lr){12-13}
        & \multicolumn{2}{c}{LSTM} & \multicolumn{2}{c}{BERT} & \multicolumn{2}{c}{T5} & \multicolumn{2}{c}{GPT-2} &\multicolumn{2}{c}{Llama 2 (senti.)}& \multicolumn{2}{c}{RNN ( Anom.)} &\multicolumn{2}{c}{Llama 2 (gene.)}
        \\
        \cmidrule(lr){2-3}  \cmidrule(lr){4-5}
        \cmidrule(lr){6-7}  \cmidrule(lr){8-9}
        \cmidrule(lr){10-11}  \cmidrule(lr){12-13}
        \cmidrule (lr){14-15}
        & & * & & * & & * & & * & & * & &* & & *\\[-0.5em]
        \midrule
Anchor  &0.43 & 0.76 & 1.87 & 1.92 & 11.06 & 10.03 & 14.05 & 8.72 & 612.78 & 276.54 & 460.30 & 371.40 & -- & --\\
LIME  &0.15 & 3.98 & 1.23 & 5.04 & 2.82 & 7.41 & 4.12 & 8.27 & 239.55 & 241.76 & 245.20 & 263.30 & 398.77 & 404.08\\
KSHAP  &0.13 & 3.97 & 1.23 & 5.45 & 3.50 & 7.93 & 4.02 & 8.08 & 289.38 & 297.90 & 267.40 & 291.40 & 424.55& 429.61\\
    \bottomrule
\end{tabular}
    % }
    }
    \caption{Average execution time (in seconds) of Anchors, LIME, and KSHAP and their \toolname-augmented version(denoted as ``*'') to explain the models in our experiments.}
\label{table:time}
\end{table*}

==> tables/userstudy.tex <==


\begin{table}[t]
    \centering
{
\setlength{\tabcolsep}{0.83mm}
    \small
\renewcommand{\arraystretch}{0.9}

% \resizebox{\columnwidth}{!}{
\begin{tabular}{@{}lcccccccccc@{}}
\toprule
\multirow{2}{*}{Methods} & \multicolumn{5}{c}{\(\mathrm{Precision}_u (\%)\)} & \multicolumn{5}{c}{\(\mathrm{Coverage}_u (\%)\)} \\
\cmidrule(lr){2-6} \cmidrule(lr){7-11} 
& T1 & T2 & T3 & T4 & T5 & T1 & T2 & T3 & T4 & T5\\
\midrule
Anchors & 70.6 & 47.4 & 18.1 & 47.4 & 57.8 & 58.0 & 44.0 & 37.0 & 37.0 & 43.5 \\
Anchors* & 81.2 & 99.4 & 73.9 & 84.1 & 97.7 & 61.9 & 69.5 & 80.5 & 71.5 & 60.5\\
\bottomrule
\end{tabular}
}
% }
\caption{Average \(\mathrm{Precision}_u\) and \(\mathrm{Coverage}_u\) of each test in the user study.}
\label{table:user_study}
\end{table}

% \begin{table*}[t]
%     \centering
% {
%     % \small
% % \renewcommand{\arraystretch}{0.8}

% \resizebox{1.5\columnwidth}{!}{
% \begin{tabular}{lccccccccccccccc}
% \toprule
% \multirow{2}{*}{Methods} & \multicolumn{5}{c}{\(\mathrm{Precision}_u (\%)\)} & \multicolumn{5}{c}{\(\mathrm{Coverage}_u (\%)\)}& \multicolumn{5}{c}{\(\mathrm{Completion\ Time\ (seconds)}\)} \\
% \cmidrule(lr){2-6} \cmidrule(lr){7-11} \cmidrule(lr){12-16}
% & T1 & T2 & T3 & T4 & T5 & T1 & T2 & T3 & T4 & T5 & T1 & T2 & T3 & T4 & T5 \\
% \midrule
% Anchors & 70.6 & 47.4 & 18.1 & 47.4 & 57.8 & 58.0 & 44.0 & 37.0 & 37.0 & 43.5 &40.0 &38.5 & 39.8 & 36.1 & 38.4\\
% Anchors* & 81.2 & 99.4 & 73.9 & 84.1 & 97.7 & 61.9 & 69.5 & 80.5 & 71.5 & 60.5 &41.9 & 36.7 &41.7 &39.8& 41.2\\
% \bottomrule
% \end{tabular}
% }
% }
% \caption{Average \(\mathrm{Precision}_u\) and \(\mathrm{Coverage}_u\) of each test in the user study.}
% \label{table:user_study_withtime}
% \end{table*}


% \begin{table}[t]
%     \centering
%     \caption{Results of the user study.}
%     \label{table:user_study}
%     {\small
%     \begin{tabular}{@{}lccccc@{}}
%         \toprule
%        \multirow{2}{*}{Method}  &T1  &T2  &T3  &T4  &T5  \\ 
%         \cmidrule{2-6}
%         & \multicolumn{5}{c}{$\mathrm{Precision_u}$ (\%)}\\
%         \midrule
%         Anchors&70.6&47.4&18.1&47.4&57.8 \\ 
%         Anchors*&81.2&99.4&73.9&84.1&97.7  \\
%         \midrule
%         &
%         \multicolumn{5}{c}{$\mathrm{Coverage_u}$ (\%)} \\
%         \midrule
%         Anchors&58.0&44.0&37.0&37.0&43.5\\
%         Anchors& 61.9&69.5&80.5&71.5&60.5 \\
%         \bottomrule
%     \end{tabular}
%     }
%     \end{table}
